Designing Robust Cyber-Defense Agents with Evolving Behavior Trees

Modern network defense can benefit from the use of autonomous systems, offloading tedious and time-consuming work to agents with standard and learning-enabled components. These agents, operating on critical network infrastructure, need to be robust and trustworthy to ensure defense against adaptive cyber-attackers and, simultaneously, provide explanations for their actions and network activity. However, learning-enabled components typically use models, such as deep neural networks, that are not transparent in their high-level decision-making leading to assurance challenges. Additionally, cyber-defense agents must execute complex long-term defense tasks in a reactive manner that involve coordination of multiple interdependent subtasks. Behavior trees are known to be successful in modelling interpretable, reactive, and modular agent policies with learning-enabled components. In this paper, we develop an approach to design autonomous cyber defense agents using behavior trees with learning-enabled components, which we refer to as Evolving Behavior Trees (EBTs). We learn the structure of an EBT with a novel abstract cyber environment and optimize learning-enabled components for deployment. The learning-enabled components are optimized for adapting to various cyber-attacks and deploying security mechanisms. The learned EBT structure is evaluated in a simulated cyber environment, where it effectively mitigates threats and enhances network visibility. For deployment, we develop a software architecture for evaluating EBT-based agents in computer network defense scenarios. Our results demonstrate that the EBT-based agent is robust to adaptive cyber-attacks and provides high-level explanations for interpreting its decisions and actions.

==> cage.tex <==
\section{CAGE EBT Details}
% overview of cage chalenge 2, 


\subsection{Environment}
% topology, 
% 3 subnets, first subnet has 5, second subnet has 4, third subnet has 4; only the enterprise servers in the second subnet matter, only operational server in the third subnet matters

The environment that we use to evaluate the effectiveness of our abstract EBT is from the CybORG Cage Challenge 2. In this environment, there is a network with three different subnets that contain hosts of varying importance. The first subnet contains five user hosts, the second subnet contains three enterprise servers and a defender host, and the third subnet contains three operational hosts and an operational server. A red agent starts at one of the user hosts in the first subnet, and its goal is to reach the operational server in the third subnet and impact its operations. A blue agent is programmatically dictated by the user, which we implement as our EBT solution. The main objective of this blue agent is to slow the red agent as much as possible, and ultimately prevent it from reaching the operational server.

% State space, 
% Different states for systems in the network include uncompromised, discovered, red agent user access, red agent root/privileged access

The different systems in a network can be in a few different states depending on the extent to which they have been compromised by a red agent. In the uncompromised state, a system has not yet been discovered by a red agent. In the discovered state, a system has been discovered by a red agent, but it has not yet take over the system. In the user access state, the red agent has basic control over the system with user level privileges. This is achieved by exploiting a remote service on the system. In the privileged access state, the red agent has complete control over a system with root privileges and is able to then continue to attack other systems. This is achieved by performing a privilege escalation on the system. The state of a system is not known by the blue agent until it explicitly observes it with an analysis action.

% action space, 
% actions for blue agent include: analyze a host, remove red agent from host (user access), deploy a decoy on a host (8 different types), restore host (red agent has root/privileged access)
% actions for red agent include:

Both the blue agent and red agent can take a variety of actions. The blue agents actions include monitor, analyze, deploy decoy, remove, and restore. The monitor action checks to see if malicious activity has occurred on a system, and occurs automatically with any other action. The analyze action checks the files on a system to see the extent to which a red agent has gained control over it. The deploy decoy action sets up a dummy service on a system that the red agent may try to exploit. If the red agent attempts to exploit this service, it will not make any progress in taking over the system, as this is simply a fake application meant to waste its turn. The remove action will remove the red agent's access to a system if it has only obtained user access over the system. The restore action will reset an entire system, which is the only way to remove the red agent if it has gained privileged access over it.

The red agent's actions include discover remote services, discover network services, exploit network services, escalate, and impact. The discover remote services actions attempts to discover other systems in the network that it can then try to gain control over. The discover network services action attempts to discover what services a host is running that may be exploitable. The exploit network services action attempts to exploit one of these vulnerable services on a system. If it succeeds in this action, it will gain user access to the system, but if it fails (such as by trying to exploit a decoy service), it will not gain any access. The escalate action attempts to perform a privilege escalation on the system so that the red agent may gain administrator access over it. The impact action is only important to the operational server, and it functionally stops the system from performing its services, rendering it useless.

% rewards, etc. 
% Red agent strategies

The red agent has two strategies that it may pursue. The first of these is Meander, in which it will explore and attempt to exploit all of the systems in a subnet before progressing to the next one. The second strategy is B-Line, in which it will attempt to reach the operational server as quickly as possible. It does this by trying to only exploiting a single system on each subnet before proceeding to the next one, until it reaches the operational server.

As a consequence of the red agent's actions, the blue agent will accrue a negative reward. The goal of the blue agent is to have the least negative reward (i.e. closest to 0) possible. The main way in which the blue agent accumulates a negative reward is through the red agent's control over different systems in the network. For each turn that the red agent has administrator access over a user host in subnet 1 or operational host in subnet 3, the blue agent will accumulate -0.1 points. Meanwhile, for each turn that the red agent has administrator access over an enterprise server in subnet 2 or the operational server in subnet 3, the blue agent will accumulate -1 point. Additionally, any time the blue agent performs a restore action, it will accrue -1 point. Finally, the most substantial action that can be taken to affect the blue agent's reward is if the red agent performs an impact action after it has gained administrator access to the operational server; this will cause the blue agent to accumulate -10 points each time it is performed.

% describe modification to the environment allowing for a red agent to switch strategies mid episode

% COPIED FROM HOTSOS PAPER

Opposed to the standard scenario in which the RedAgent selects one strategy for the entirety of an episode, our scenario sees the \textit{RedSwitch} agent change from a \textit{Meander} to a \textit{BLine} strategy. This is set to randomly occur between timesteps 10-30, simulating how an attacker may change their strategy based on information of the network structure that they can quickly obtain.

Two autonomous agents were trained based on the \textit{Meander} and \textit{BLine} strategies using a PPO policy. The policies consist of actor-critic neural networks with the actor and critic networks containing 1 layer of size 64.  Both of these policies were trained for 100k observations with 1000 episodes each in a non-deterministic manner. This was done using a multi-layered perceptron developed by the \textit{CardiffUni} team. Training was done in order to minimize the negative reward received by the blue agent from allowing the red agent to take certain actions and reach various hosts. The blue agent receives a reward of -0.1 per turn for each user and operational host (excluding user host 0) the red agent has access to. A reward of -1 per turn is received for each enterprise and operational server the red agent has access to, or if a blue agent performs a restore operation. If the red agent performs an impact action on the operational server, the blue agent receives a reward of -10 per turn. Since these rewards are negative, an optimal solution should be closer to 0, indicating better success at mitigating a red agent attack.

\subsection{Cardiff Solution}
% Cardiff uni solution described here

% overview of method and why their solution is better than others (most likely to do with reduced action space and decoy selection)

% GitHub URL: https://github.com/john-cardiff/-cyborg-cage-2
The structure of our initial CAGE EBT is modelled from the control flow of the \textit{CardiffUni} solution. Their solution won the CAGE Challenge 2, as it was able to attain the lowest reward out of all solutions. In their solution, they use a combination of a reduced action space, along with greedy decoy selection. The reduced action space was selected through observation of which behaviors appeared most important and seemed to have the largest impact on reducing the effectiveness of the red agent. Meanwhile, the greedy decoy selection was performed with the intent of having the blue agent attempt to deploy the best decoy possible for each host. This list of decoys also appears to have been selected through observation and testing through greedy searches.

% describe reduced action space

The reduced action space sees the overall action space of 145 actions reduced to only 52 actions. Part of this reduction was by eliminating actions that are performed on non-essential systems that are not targeted by the B-Line agent, leaving the action space to only deal with user hosts 1-4, enterprise servers 0-2, the defender, and the operational server. For each of these systems, only the analyze, remove, and restore actions are available, in addition to a few selected decoys for each systems. Enterprise servers 1-2 and user host 4 have 1 decoy available, user host 3 has 2 decoys available, and the remaining systems that are used in the reduced action space are each given 4 decoys available. 

% training algorithm description (PPO, number of policies learned) 

% describe neural net architecture details and different hyperparameters (episodes, number of layers, input/output)

The model that the \textit{CardiffUni} solution is based on is a PPO policy. A policy is learned for each of the B-Line and Meander agents. Each policy contains an actor and a critic, each of which contain 3 hidden layers that use linear blocks with a ReLU after the first 2 hidden layers. The output of the actor has a softmax applied, while the output of the critic is reduced to a single vector. They train for 100000 episodes with 100 timesteps each with Adam as their optimizer. They also use a learning rate of 0.002, gamma of 0.99, and betas of 0.9 and 0.99.

\subsection{Learned Switching}
% learned switching approach overview

% describe LSTM training algorithm: Collect data from oracle that correclty determines strategy, then train in a supervised manner with binary cross entropy loss (see hotsos paper)

% describe neural net architecture details and different hyperparameters (epochs, dataset size, input/output, number of layers)

% COPIED FROM HOTSOS PAPER

An LSTM model was trained in order to carry out the strategy switching. This model was trained with a window size of 5 over 5 epochs (3000 optimization iterations) with 100k observations (1000 episodes) using supervised Binary Cross Entropy loss. Observations are collected using an oracle that correctly labels each strategy, Meander or BLine. The supervised loss is used to optimize the predicted label of the strategy from the LSTM with the correct labelling from the oracle using a window of observations. The LSTM model consists of a neural network with 2 layers of size 100. The learning rate used was $1e-3$.

\subsection{Behavior Mapping}
% Describe how the high-level behaviors I described in the Cyber BT Behaiovrs section map to actions in CAGE

The behaviors developed for the Cyber BT map neatly to the CAGE Challenge 2 environment. The \textit{GetAnalyzeAction!} action corresponds to the analyze action in CAGE. The \textit{GetDetectorAction!} action corresponds to the deploy decoy action in CAGE. The \textit{GetMitigateAction!} action can correspond to both the remove and restore actions in CAGE.

\subsection{Behavior Tree Structure}

% identify learning-enabled components and their relations to the behaviors

% describe the execution process of this BT (control flow; how behaviors transition between each other)

The EBT contains two learning enabled components. These include the PPO Agent and Learned Switch models hat were previously discussed. The tree uses a sequence node as the root node to ensure that every one of its child nodes executes until one of them files. Its child nodes include fallback nodes and action nodes.

The first fallback tests to see if the strategy should be changed. If a condition is met, then it will perform a strategy switch, otherwise nothing will happen. This uses the Learned Switch model in order to determine if the strategy should be changed. The next node uses the other learned model, the PPO agent, to determine the action that the blue agent should take. Following this a fallback node is used to test if the action selected is an analyze. If so, the analyze action is performed. The next node is another fallback node that detects if the action selected is to deploy a decoy. If so, a decoy is selected and deployed using the greedy decoy algorithm. After this, there are two action nodes that check the same analyze and decoy conditions that were part of the fallback nodes. This is because if one of these is the action, then the condition will also fail here as it did in its fallback node, causing the sequence node to finish execution. But if both of these nodes succeed, meaning that the action is neither of these, then the remove decoys action is performed, which corresponds to a restore action.

\subsection{Results}

% Overview of what evaluation metrics and comparision we will make (determine if ebt is able to react to different red strategies) Same idea as the hotsos paper here

% Describe training configs
% Cardiff
% Oracle
% LearnedSwitch

% Demonstrate with plots/tables that original cardiff and ebt have similar to exactly the same performance when using the 

% Demonstrate with plots/tables that the ebt with learned switching policy is more robust than cardiff's fixed strategy selection policy.

% Descirbe with image and text the explainable nature of Ebts

% COPIED FROM HOTSOS
In % Insert figure here Figure~\ref{fig:reward_results} 
, our LearnedSwitch solution shows a significant improvement over the CardiffUni solution. The CardiffUni solution managed an average cumulative reward of -16.6, while our LearnedSwitch solution achieved an average cumulative reward of only -3.51.  This indicates that a strategy switch from the cyber operator is imperative to properly defend against a red agent that can switch strategies; solely detecting its strategy at the beginning of an episode is not sufficient. It should be noted that this solution did not see a noticeable drop in performance in the range of timesteps in which the red agent could change strategies. This highlights our solution as being resilient to a sudden change in strategy, as it can rapidly detect and adapt to it.

The performance for the cyber-firefighter BT is the exact same (see graphs in figs section).

\subsection{Conclusion}
% Give high level summary of what you just described for this section
% Important conclusions from the results about ebts robustness and interpretability

% Potential future applications you see from this work. Challenges? Limitations?

==> gp.tex <==
\section{Learning Structure}
% overview of learning BT structure
To learn the optimal structure of an EBT for autonomous cyber-defense requires an algorithm to construct BTs from high-level task knowledge. We utilize genetic programming (GP), an algorithm designed to build optimal solutions given a set of components, to build BTs given a set of behaviors.   

GP requires a fitness function to evaluate the performance of a constructed BT. As such, we develop an abstract environment, that translates to cyber-security, to simulate and evaluate a BT structure. Also, the abstract environment allows for computationally efficient simulation of a BT structure instead of relying on computationally heavy simulation in a realistic environment. The computationally efficient abstract environment in tandem with genetic programming for learning is used as our approach for constructing the EBT. 

In the following, we first describe the abstract environment to evaluate the BT construction. Then, we formalize the behaviors used to construct the EBT and map to the abstract environment. Finally, we describe the GP algorithm that will utilize the behaviors and environment to construct the optimal EBT. 

\subsection{Cyber-Firefighter Abstract Environment}
% cyberfire overview and inspiration
The abstract environment \textit{Cyber-Firefighter} is a partially-observable pursuit-evasion game where a defender must contain an attacker from spreading on a network. The pursuit-evasion game is inspired by \textit{Firefighter}, a game where a "firefighter" (defender) must optimally contain a spreading "fire" (attacker) in a network of "trees" (nodes) using full knowledge of the "fire" movements and "fire retardant" to block the spread. The game terminates when the "fire" can no longer spread to new "trees".

% Whats different about cyber-firefighter
In \textit{Cyber-Firefighter}, the objective remains the same, but to make the game similar to cyber-defense on a computer network, we do not have full knowledge of the "fire" (attacker) movements. Therefore,  we re-frame the problem as partially observable and include two new actions to reveal information in the environment. The defender will be able to deploy "drones" (detectors) to reveal the "fire" if it spreads into a "drone" detection zone. Also, the defender can activate a "drone" (perform analysis) to increase the detection zone and gain further information from the environment. Once information is revealed on the "trees" the "fire" has spread to, "fire retardant" can be placed to block the spread.

% Formal definitions of environment and agent actions
More formally, the \textit{Cyber-Firefighter} environment is defined as a network $G: (V, E)$ with neighbors for each "tree" node vertex $N(v) = \{u\ |\ (v, u) \in E,\ v, u \in V\}$. The induced neighbor subgraph, $N_r(v)$, is the subgraph with nodes up to a radius $r$ from node $v$. Terms used to describe transitions in the environment are as follows:
\begin{itemize}
    \item Fire Source $v_f \in V$  
    \item Burn Time $T_{burn} \in \mathbb{R}$  
    \item Burn Amount $B: v \rightarrow b$ where $b \in [0, T_{burn}]$   
    \item Drone Status $D: v \rightarrow d, d \in [nodrone, inactive, active]$   
    \item Drone Search Range $r$  
    \item Retardant Nodes $R$   
    \item Visible Nodes $I$
\end{itemize}
The objective of the "firefighter" is to limit the number of nodes with the maximum burn amount: $v \in V | B(v) = T_{burn}$. The objective of the "fire" is the opposite, to maximize the number of nodes with maximum burn amount.  

At each timestep, a single action can be taken by the "fire" (attacker) and the "firefighter" (defender). The "fire" has one action, "burn", defined as follows:
\begin{align*}
    &B(u) = min(B(u) + 1, T_{burn}), \forall u \in M \\ \text{ where }
    &M = \{u\ |\ u \in N_1(v), \ B(v) = T_{burn},\ u \notin R,\ v, u \in V\}
\end{align*}
The constraint ensures that only nodes that are fully burned $B(u) = T_{burn}$ will spread to neighbors without retardant. The neighboring nodes will take $T_{burn}$ and at that point they will also spread to neighboring nodes.

The intuition behind the delay is to allow time for the firefighters to find the fire. Otherwise, if trees burned every timestep, this would become a much more challenging problem. 

The "firefighter" has three potential actions:
\begin{itemize}
    \item Deploy Drone $D(v) = inactive$ then update visibility $I = I\ \cup\ N_0(v)$
    \item Activate Drone Area Search: if $D(v) = inactive$ then $D(v) = active$ then update visibility $I = I\ \cup\ N_r(v)$
    \item Place Fire Retardant $R = R\ \cup\ \{v\ |\ v\in V, v \in I, B(v) \neq T_{burn}\}$
\end{itemize}

We separate deploying drones and area search into two steps. Deploying a drone will only gain visibility for the vertex the drone is deployed on. An area search can then be activated that gains visibility of neighboring nodes. The two steps allows for players to develop strategies to consume time to reveal more information (vertex visibility) via area search or to move towards placing fire retardant after deploying a drone. 

Two constraints are added to the placing of fire retardant. Fire retardant can only be placed on visible nodes. We want to instill confident actions in an agent. Also, Fire retardant can only be placed on non-burned nodes $v \in V | B(v) = 0$.

After a certain number of timesteps, the game terminates when the "fire" cannot spread further. The condition is formalized as the burn amounts not changing between two timesteps,  $B_{t-1}(v) = B_{t}(v), \forall v \in V$.

\subsection{Cyber BT Behaviors}

To construct a BT requires a set of behaviors as building blocks. The behaviors should be generalizable and should map to our abstract environment and to a realistic cyber-security environment (CybORG).  We define five action behaviors, to allow the BT to select defense strategies (\textit{SelectStrategy!}, select a defense operation using a strategy (\textit{GetMetaAction!}), and enact three defense operations. 

The first defense operation, (\textit{GetDetectorAction!}), deploys a detection mechanism in the environment to alert of local adversarial activity. The second, \textit{GetMitigateAction!}, prevents an adversary from achieving their objective, such as blocking adversarial movement or restoring a network node to previously "good" state. The final operation, \textit{GetAnalysisAction!}, monitors or analyzes the environment retrieving new information otherwise unknown to the agent. 

Furthermore, there are four condition behaviors. One for each defense operation behavior, to ensure it is only enacted when chosen using \textit{GetMetaAction!} and one for \textit{SelectStrategy!} to ensure the strategy is only selected or shifted when necessary.

% behavior mapping
\subsection{Abstract Behavior Mapping}
To construct BTs for execution in the \textit{Cyber-Firefighter} environment, we map the defined BT behaviors to actionable behaviors in the environment. The three defense operations map to the three "firefighter" actions. Each defense operation determines a node to deploy a drone (\textit{GetDetectorAction!}), activate a drone for further visibility analysis (\textit{GetAnalysisAction!}), and place fire retardant to block the fire spread (\textit{GetMitigateAction!}. \textit{GetMetaAction!} selects which operation to perform using a strategy. In this paper, the strategy defines a state-action policy for choosing operations based on the current state of the fire and visibility of network. \textit{SelectStrategy!} determines the appropriate strategy to enact based on the state of the environment. For example, a strategy could be to repeat the process of: deploy a drone, activate the drone, then place retardant.


\subsection{Genetic Programming for BTs}
To learn the optimal structure of the EBT, we use GP combined with suboptimal baseline BTs. The inputs to the GP are the pre-defined BT nodes for the \textit{Cyber-Firefighter} environment and a baseline BT that only considers strategy selection. The abstract environment will be used for evaluation and computation of a fitness value for optimizing towards an efficient BT that mitigates the attacker spread on the network.

More specifically, the GP algorithm is initialized with the behavior set execution nodes and control nodes defined and randomly generated BTs from the behavior set. The intention of the baseline BT is to provide a starting representation to encourage expansion and enhance training efficiency. After initialization, the GP algorithm selects, breeds, and evaluates BTs for a fixed number of generations using a fitness function, ultimately computing a solution that maximizes the fitness.

The fitness function is the primary component in GP that drives the definition of the optimal BT. We consider the "fire" impact, the visibility of the network, and the size of BT nodes as a fitness function for the \textit{Cyber-Firefighter} environment. We define the fitness function as 

\begin{equation*}
    F(x) = c_v |I| - c_l |x| -c_f \sum_0^{T_{f}}| \{v \in V \ | \ B(v) = T_{burn}\} |
\end{equation*}

where $|x|$ is the number of nodes in the BT. The "fire" impact is measured by the sum of number of nodes with max burn amount at each timestep. This encourages a compact and efficient BT that can mitigate adversarial activity while revealing information from the environment to make informed decisions.

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{figs/gp/baseline_bt.png}
    \caption{Baseline BT considering only strategy selection}
    \label{fig:baseline_bt}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figs/gp/gpbt.png}
    \caption{EBT Structure for Autonomous Cyber-Defense}
    \label{fig:bt_structure}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{figs/gp/gptbt_training.pdf}
    \caption{GP Fitness}
    \label{fig:gp_training}
\end{figure}

\subsection{Evaluation}

For evaluation of learning the structure of the EBT, we consider a comparison of multiple BT structures and their respective performance in the abstract environment.

The \textit{Cyber-Firefighter} environment is setup as an Erdos-Renyi (ER) graph with 10 nodes and a probability of 0.2 for edge connection with a constraint that the graph must be connected, otherwise the "fire" could not spread to all nodes. For each simulation a new ER graph will be constructed with a fixed fire source $v_f = 0$. $T_{burn}=4$ to alleviate the challenge of partial observability, providing more time for an agent to gain visibility and mitigate.

The GP algorithm is initialized with 16 BTs and the baseline BT in Figure~\ref{fig:baseline_bt}. The baseline BT is \textit{boosted} through the inclusion in each generation and preference towards crossover and mutation. In each generation a BT is represented using a hierarchical list of strings representation as the BT, which can then be directly converted to an executable BT for evaluation. The string representation allows for simple operations to update and add new behaviors before execution. The algorithm is executed for 10 trials of 200 generations with approximately 5000 simulation runs (episodes) recorded with the best fitness for each generation stored. We compare the fitness of the GP BTs, the baseline BT, and an expert manually crafted BT.

The results are shown in Figure~\ref{fig:gp_training}. The BT fitness improves from the baseline up to the Expert BT. The best computed BT from the trials is shown in Figure~\ref{fig:bt_structure} which achieves an fitness of $-19.45$, the same fitness as the Expert BT. Therefore, we conclude that we can
learn the structure of a BT to achieve an abstract cyber-security task with performance similar to a BT constructed 
manually with expert knowledge.

